Dynamic Named Entity Recognition

Named Entity Recognition (NER) is a challenging and widely studied task that involves detecting and typing entities in text. So far,NER still approaches entity typing as a task of classification into universal classes (e.g. date, person, or location). Recent advances innatural language processing focus on architectures of increasing complexity that may lead to overfitting and memorization, and thus, underuse of context. Our work targets situations where the type of entities depends on the context and cannot be solved solely by memorization. We hence introduce a new task: Dynamic Named Entity Recognition (DNER), providing a framework to better evaluate the ability of algorithms to extract entities by exploiting the context. The DNER benchmark is based on two datasets, DNER-RotoWire and DNER-IMDb. We evaluate baseline models and present experiments reflecting issues and research axes related to this novel task.

==> tables/RotoWire_task1_results.tex <==
    \begin{subtable}{0.5\textwidth}
     \centering
\footnotesize
    \begin{tabular}{lccccc}
    \hline
    \textbf{Label} & \textbf{Model} & \textbf{Set} & \textbf{Precision} & \textbf{Recall}& \textbf{F1}  \\
    \hline
        \multirow{8}{*}{Looser} & \multirow{4}{*}{Baseline}     & Seen        & 0.81 & \textbf{0.77} & \textbf{0.79} \\
                                 &                              & Seen/Unseen & 0.77 & \textbf{0.74} & \textbf{0.75} \\
                                 &                              & Unseen      & 0.76 & \textbf{0.73} & \textbf{0.74} \\
                                 &                              & All         & 0.77 & \textbf{0.74} & \textbf{0.76} \\
                                 \cline{2-6}
                                 & \multirow{4}{*}{BaselineCLS} & Seen        & \textbf{0.89} & 0.66 & 0.75 \\
                                 &                              & Seen/Unseen & \textbf{0.84} & 0.61 & 0.71 \\
                                 &                              & Unseen      & \textbf{0.85} & 0.58 & 0.69 \\
                                 &                              & All         & \textbf{0.85} & 0.61 & 0.71 \\
                                \cline{2-6} 
        \multirow{8}{*}{Winner}  & \multirow{4}{*}{Baseline}    & Seen        & \textbf{0.80} & 0.84 & 0.82 \\
                                 &                              & Seen/Unseen & \textbf{0.78} & 0.81 & 0.79 \\
                                 &                              & Unseen      & \textbf{0.78} & 0.81 & 0.79 \\
                                 &                              & All         & \textbf{0.79} & 0.81 & 0.80 \\    
                                \cline{2-6}
                                 & \multirow{4}{*}{BaselineCLS} & Seen        & 0.75 & \textbf{0.92} & \textbf{0.83} \\
                                 &                              & Seen/Unseen & 0.73 & \textbf{0.90} & \textbf{0.81} \\
                                 &                              & Unseen      & 0.72 & \textbf{0.91} & \textbf{0.81} \\
                                 &                              & All         & 0.73 & \textbf{0.91} & \textbf{0.81} \\

    \hline
    \end{tabular}
    \caption{Label statistics on rotowire}
    \end{subtable}
   \begin{subtable}{0.5\textwidth}
   \centering
    \begin{tabular}{lccc}
    \hline
    \textbf{Model} & \textbf{Set} & \textbf{BCELoss} & \textbf{Accurary}   \\
    \hline
        \multirow{4}{*}{Baseline}   & Seen        & $0.557\pm035$ & $0.832\pm0.006$  \\
                                    & Seen/Unseen & $0.703\pm0.028$ & $0.795\pm0.005$  \\
                                    & Unseen      & $0.716\pm0.028$ & $0.790\pm0.005$  \\
                                    & All         & $0.680\pm0.028$ & $0.801\pm0.004$  \\
                                 \hline
        \multirow{4}{*}{BaselineCLS}  & Seen        & $\textbf{0.496}\pm0.052$ & $\textbf{0.840}\pm0.010$ \\
                                      & Seen/Unseen & $\textbf{0.623}\pm0.048$ & $\textbf{0.805}\pm0.011$ \\
                                      & Unseen      & $\textbf{0.642}\pm0.029$ & $\textbf{0.797}\pm0.006$ \\
                                      & All         & $\textbf{0.606}\pm0.046$ & $\textbf{0.810}\pm0.009$ \\

    \hline
    \end{tabular}
        \caption{Overall statistics on rotowire}

    \end{subtable}
   


==> tables/imdb_results.tex <==
%======================= CNET ===============================
\begin{subtable}{\textwidth}
    \footnotesize
    \centering
    \resizebox{\textwidth}{!}{

    \begin{tabular}{|c|c||ccc|ccc|ccc|ccc|c|}
    \hline
    \multirow{3}{*}{\textbf{Models}}& \multirow{3}{*}{\textbf{Set}} & \multicolumn{13}{c|}{CNET} \\
    \cline{3-15}
                                 &                               & \multicolumn{3}{c}{1}             & \multicolumn{3}{c}{2}      & \multicolumn{3}{c}{3}        & \multicolumn{3}{c}{4}       & All       \\ 
                                 &                               & P         & R             & F1    & P         & R      & F1    & P      & R          & F1     & P    & R           & F1     &\mu F1    \\
    \hline
    \multirow{2}{*}{BERT-Linear} & Seen                          & 0.83      & 0.87          & 0.85  & 0.61      & 0.67   & 0.64  & 0.64   & 0.68       & 0.66   & 0.75 & 0.42        & 0.54   & 0.67 \\
                                 & Unseen                        & 0.71      & 0.75          & 0.73  & 0.39      & 0.44   & 0.42  & 0.40   & 0.45       & 0.42   & 0.39 & 0.17        & 0.23   & 0.45 \\
    \hline
    \multirow{2}{*}{BERT-CLS}    & Seen                          & 0.84      & 0.87          & 0.86  & 0.63      & 0.69   & 0.65  & 0.68   & 0.67       & 0.67   & 0.70 & 0.52        & 0.59   & 0.69 \\
                                 & Unseen                        & 0.71      & 0.76          & 0.73  & 0.40      & 0.43   & 0.42  & 0.40   & 0.41       & 0.40   & 0.35 & 0.22        & 0.27   & 0.46    \\
    \hline
    \end{tabular}
    }
    \caption{Comparative results on the DNER-IMDb dataset for the DNET task.}
\end{subtable}


%======================= CNER ===============================
\centering
\begin{subtable}{\textwidth}
    \footnotesize
    \centering
    \resizebox{\textwidth}{!}{

    \begin{tabular}{|c|c||ccc|ccc|ccc|ccc|ccc|c|}
    \hline
    \multirow{3}{*}{\textbf{Models}}& \multirow{3}{*}{\textbf{Set}} & \multicolumn{16}{c|}{CNER} \\
    \cline{3-18}
                                 &                               & \multicolumn{3}{c}{Entity}        & \multicolumn{3}{c}{1}      & \multicolumn{3}{c}{2}        & \multicolumn{3}{c}{3}        & \multicolumn{3}{c}{4}       & All       \\ 
                                 &                               & P         & R             & F1    & P         & R      & F1    & P      & R          & F1     & P    & R           & F1      & P    & R           & F1     &\mu F1    \\
    \hline
    \multirow{2}{*}{BERT-Linear} & Seen                          & 0.52      & 0.84          & 0.58  & 0.71      & 0.77   & 0.74  & 0.39   &  0.36      & 0.37   & 0.15 &  0.08       & 0.09    & 0.41 & 0.61        & 0.49    & 0.36      \\
                                 & Unseen                        & 0.51      & 0.83          & 0.56  & 0.67      & 0.70   & 0.68  & 0.35   &  0.32      & 0.34   & 0.14 &  0.07       & 0.08    & 0.34 & 0.51        & 0.41    &0.31\\
    \hline
    \multirow{2}{*}{BERT-CLS}    & Seen                          &  0.54     & 0.87          & 0.60  &  0.40     & 0.77   & 0.44  & 0.39   &  0.43      & 0.41   & 0.34 &  0.14       &  0.20   & 0.44 &  0.59       &  0.50   & 0.37   \\
                                 & Unseen                        &  0.52     & 0.85          & 0.58  &  0.36     & 0.69   & 0.40  & 0.34   &  0.36      & 0.35   & 0.28 &  0.13       & 0.17    & 0.36 & 0.48        &  0.41   & 0.32      \\
    \hline
    \multirow{2}{*}{BERT-CRF}    & Seen                          &  0.97     & 0.92          & 0.94  &  0.77     &  0.84  & 0.80  & 0.47   &  0.53      & 0.50   & 0.54 &  0.50       &  0.52   & 0.37 &  0.08       &  0.13   &  0.60 \\
                                 & Unseen                        &  0.96     & 0.89          & 0.92  &  0.68     &  0.76  & 0.72  & 0.41   &  0.43      & 0.42   & 0.41 &  0.38       &  0.39   & 0.30 &  0.05       &  0.09   &  0.52   \\
    \hline
    \multirow{2}{*}{BERT-CLS-CRF}& Seen                          &  0.89     & 0.91          & 0.90  &   0.71    &  0.84  & 0.77  &  0.38  &   0.53     &  0.44  & 0.51 &   0.44      & 0.47    & 0.32 &   0.04      &  0.07   & 0.56  \\
                                 & Unseen                        &  0.88     & 0.89          & 0.88  &   0.63    &   0.76 &  0.68 &  0.34  &   0.44     &  0.38  & 0.41 &  0.35       &  0.38   & 0.27 &  0.03       &   0.05  &  0.48   \\
    \hline
    \end{tabular}
    }
    \caption{Comparative results on the DNER-IMDb dataset for the DNER task.}
\end{subtable}


==> tables/imdb_results_acc.tex <==

%======================= CNER ===============================

    \footnotesize
    %\centering
    \begin{tabular}{|c|c||c|c|}
    \hline
    \multirow{2}{*}{\textbf{Models}} & \multirow{2}{*}{\textbf{Set}} & \multicolumn{2}{c|}{\mu F1} \\
                                 &              & CNET          &  CNER          \\
    \hline  
    \multirow{4}{*}{BERT-Linear} & Seen         &  0.71          & 0.30      \\
                                 & Unseen       &  0.54          & 0.21      \\
                                 & All          &  0.58          & 0.22      \\
    \hline
    \multirow{4}{*}{BERT-CLS}    & Seen         &  0.73          &  0.36     \\
                                 & Unseen       &  0.53          &   0.25    \\
                                 & All          &  0.56          &  0.27      \\
    \hline
    \multirow{4}{*}{BERT-CRF}    & Seen         &   -            &  0.69     \\
                                 & Unseen       &  -             &  0.48     \\
                                 & All          &    -           &  0.51     \\
    \hline
    \multirow{4}{*}{BERT-CLS-CRF}& Seen         &   -            &  0.57      \\
                                 & Unseen       &    -           &  0.43       \\
                                 & All          &   -            &  0.45      \\
    \hline
    \end{tabular}


==> tables/imdb_task1_results.tex <==
    \begin{subtable}{1\textwidth}
     \centering

    \begin{tabular}{lccccc}
    \hline
    \textbf{Label} & \textbf{Model} & \textbf{Set} & \textbf{Precision} & \textbf{Recall}& \textbf{F1}  \\
    \hline
        \multirow{6}{*}{1}       & \multirow{4}{*}{Baseline}    & Seen        & 0.80 & \textit{0.87} & \textit{0.83} \\
                                 &                              & Unseen      & 0.73 & \textit{0.79} & \textit{0.76}\\
                                 &                              & All         & 0.74 & \textit{0.81} & \textit{0.78} \\
                                \cline{3-6}
                                 & \multirow{4}{*}{BaselineCLS} & Seen        & \textit{0.81} & 0.85 & \textit{0.83} \\
                                 &                              & Unseen      & \textit{0.74} & 0.76 & 0.75 \\
                                 &                              & All         & \textit{0.75} & 0.78 & 0.77 \\
                                \cline{2-6} 
        \multirow{6}{*}{2}       & \multirow{4}{*}{Baseline}    & Seen        & \textit{0.61} & \textit{0.63} & \textit{0.62} \\
                                 &                              & Unseen      & \textit{0.42} & 0.42 & 0.42\\
                                 &                              & All         & 0.46 & 0.47 & 0.47 \\
                                \cline{3-6}
                                 & \multirow{4}{*}{BaselineCLS} & Seen        & 0.60 & 0.64 & \textit{0.62} \\
                                 &                              & Unseen      & \textit{0.42} & \textit{0.44} & \textit{0.43} \\
                                 &                              & All         & \textit{0.47} & \textit{0.49} & \textit{0.48} \\   
                                \cline{2-6} 
        \multirow{6}{*}{3}       & \multirow{4}{*}{Baseline}    & Seen        & 0.64 & 0.63 & \textit{0.64 \\
                                 &                              & Unseen      & 0.39 & 0.42 & 0.40\\
                                 &                              & All         & 0.45 & 0.47 & 0.46 \\
                                \cline{3-6}
                                 & \multirow{4}{*}{BaselineCLS} & Seen        & \textit{0.65} & \textit{0.64} & \textit{0.64} \\
                                 &                              & Unseen      & \textit{0.40} & \textit{0.45} & \textit{0.42} \\
                                 &                              & All         & \textit{0.46} & \textit{0.50} & \textit{0.48}\\     
                                \cline{2-6} 
        \multirow{6}{*}{4}       & \multirow{4}{*}{Baseline}    & Seen        & 0.68         & 0.48         & 0.56 \\
                                 &                              & Unseen      & \textit{0.36} & \textit{0.23} & \textit{0.28} \\
                                 &                              & All         & 0.44         & 0.29         & \textit{0.35} \\
                                \cline{3-6}
                                 & \multirow{4}{*}{BaselineCLS} & Seen        & \textit{0.74} & \textit{0.56} & \textit{0.63} \\
                                 &                              & Unseen      & \textit{0.36} & \textit{0.23} & \textit{0.28} \\
                                 &                              & All         & \textit{0.46} & \textit{0.31} & \textit{0.37} \\     

    \hline
    \end{tabular}
    \caption{Label statistics on rotowire}
    \end{subtable}
   \begin{subtable}{0.5\textwidth}
   \centering
    \begin{tabular}{lccc}
    \hline
    \textbf{Model} & \textbf{Set} & \textbf{BCELoss} & \textbf{Accurary}   \\
    \hline
        \multirow{4}{*}{Baseline}   & Seen        & 1.255\pm0.048 & 0.577\pm0.004  \\
                                    & Unseen      & 2.296\pm0.110 & 0.346\pm0.005  \\
                                    & All         & 2.05\pm0.090 & 0.400\pm0.005  \\
                                 \hline
        \multirow{4}{*}{BaselineCLS}  & Seen        & \textit{1.194\pm0.092 & \textit{0.580\pm0.018 \\
                                      & Unseen      & \textit{2.164\pm0.109 & \textit{0.354\pm0.006 \\
                                      & All         & \textit{1.94\pm0.101 & \textit{0.406\pm0.005 \\

    \hline
    \end{tabular}
        \caption{baseline results on CNET-ImDB}

    \end{subtable}
   


==> tables/label_coherence.tex <==
    % \begin{subtable}{1\textwidth}
    % \footnotesize
    % \centering
    %     \begin{tabular}{lccccc}
    %     \hline
    %     \textbf{Set} & \textbf{Total Entity mentions} & \textbf{Incoherent Entity GT}   \\
    %     \hline
    %      Seen           & 239   & 13 (5.439\%)    \\
    %      Seen//Unseen   & 1165  & 54 (4.635\%)     \\
    %      Unseen         & 190   & 15 (2.631\%)     \\
    %      All            & 1594  & 72 (4.516\%)  \\
    %     \hline
    %     \end{tabular}
    %     \caption{Incoherence statistics on \textbf{CNET-RotoWire} grount truth.}
    % \end{subtable}
    
    \begin{subtable}{1\textwidth}
    \footnotesize
    \centering
        \begin{tabular}{lccccccc}
        \hline
        \textbf{Model} & \textbf{Set} & \textbf{Ground truth} &\textbf{All} & \textbf{Winners} & \textbf{Losers}  \\
        \hline
         \multirow{4}{*}{Bert-Linear} & Seen &             13/239 (5.44\%) & 40/226 (17.69\%)     & 19/130 (14.61\%)    & 21/96 (21.87\%)    \\
                                      & Seen/Unseen  & 54/1165 (4.64\%)   & 232/1111 (20.88\%)   & 119/679 (17.52\%)   & 113/432 (26.15\%)   \\
                                      & Unseen  & 15/190 (2.63 \%)         & 38/185 (20.54\%)     & 23/128 (17.96\%)    & 15/57 (26.31\%)    \\
                                      &  All  &72/1594 (4.52\%)           & 310/1522 (20.36\%)   & 161/937 (17.18\%)   & 149/585 (25.47\%)  \\
        \hline
        \multirow{4}{*}{Bert-CLS}     & Seen&             13/239 (5.44\%)  & 30/226 (13.27\%)     & 12/130 (9.23\%)    & 18/96 (18.75\%)    \\
                                      & Seen/Unseen  & 54/1165 (4.64\%)   & 203/1111 (18.27\%)   & 91/679 (13.40\%)   & 112/432 (25.92\%)   \\
                                      & Unseen  & 15/190 (2.63 \%)         & 20/185 (10.81\%)     & 10/128 (7.81\%)    & 10/57 (17.54\%)    \\
                                      &  All  &72/1594 (4.52\%)           & 253/1522 (16.62\%)   & 113/937 (12.05\%)  & 140/585 (23.93\%)  \\
        \hline

        \end{tabular}
        \caption{Inconsistency analysis statistics on \textbf{CNET-RotoWire}. Entity with a single mention are ignored.}
    \end{subtable}
    
    
    
    %     \begin{subtable}{1\textwidth}
    % \footnotesize
    % \centering
    %     \begin{tabular}{lcccccc}
    %     \hline
    %     \textbf{Model} & \textbf{Set} & \textbf{total multiple mention / incoherence} & \textbf{Winner mention / incoherence} & \textbf{Loser mention / incoherence}  \\
    %     \hline
    %      \multirow{4}{*}{Bert-Linear} & Seen             & 40/226 (17.69\%)     & 19/130 (14.61\%)    & 21/96 (21.87\%)    \\
    %                                   & Seen//Unseen     & 232/1111 (20.88\%)   & 119/679 (17.52\%)   & 113/432 (26.15\%)   \\
    %                                   & Unseen           & 38/185 (20.54\%)     & 23/128 (17.96\%)    & 15/57 (26.31\%)    \\
    %                                   &  All             & 310/1522 (20.36\%)   & 161/937 (17.18\%)   & 149/585 (25.47\%)  \\
    %     \hline
    %     \multirow{4}{*}{Bert-CLS}     & Seen             & 30/226 (13.27\%)     & 12/130 (9.23\%)    & 18/96 (18.75\%)    \\
    %                                   & Seen//Unseen     & 203/1111 (18.27\%)   & 91/679 (13.40\%)   & 112/432 (25.92\%)   \\
    %                                   & Unseen           & 20/185 (10.81\%)     & 10/128 (7.81\%)    & 10/57 (17.54\%)    \\
    %                                   &  All             & 253/1522 (16.62\%)   & 113/937 (12.05\%)  & 140/585 (23.93\%)  \\
    %     \hline

    %     \end{tabular}
    %     \caption{Incoherence statistics on \textbf{CNET-RotoWire}. Entity with a single mention are ignored}
    % \end{subtable}
    
    % \begin{subtable}{1\textwidth}
    % \footnotesize
    % \centering
    %     \begin{tabular}{lccccccc}
    %     \hline
    %     \textbf{Set} & \textbf{Total Entity mentions} & \textbf{Incoherent Entity GT}  \\
    %     \hline
    %      Seen           & 1975 & 0 (0.0\%)   \\
    %      Unseen         & 6319 & 2 (0.031\%) \\
    %      All            & 8294 & 2 (0.024\%) \\
    %     \hline
    %     \end{tabular}
    %     \caption{Incoherence statistics on \textbf{CNET-ImDB} grount truth.}
    % \end{subtable}
    
    
    \begin{subtable}{1\textwidth}
    \footnotesize
    \centering
        \begin{tabular}{lccccccc}
        \hline
        \textbf{Set} & \textbf{Movies} & \textbf{Ground truth} & \textbf{All} & \textbf{Label 1} & \textbf{Label 2} & \textbf{Label 3} & \textbf{Label 4}  \\
        \hline
         \multirow{4}{*}{Bert-Linear} & Seen   &  0/1975 (0\%)       & 143/1975 (7.24\%)    & 34/759 (4.47\%)     & 30/478 (6.27\%)     & 54/486 (11.11\%)     & 25/252 (9.92\%)\\
                                      & Unseen &  2/6319 (0.31\%)        & 546/6317 (8.64\%)    & 138/2465 (5.59\%)   & 160/1591 (10.05\%)  & 170/1414 (12.02\%)   & 78/847 (9.20\%)  \\
                                      & All   & 2/8294 (0.024\%)         & 689/8292 (8.30\%)    & 172/3224 (5.33\%)   & 190/2069 (9.18\%)   & 224/1900 (11.78\%)   & 103/1099 (9.37\%) \\
        \hline
         \multirow{4}{*}{Bert-CLS}    & Seen   &  0/1975 (0\%)        & 99/1975 (5.01\%)    & 28/759 (3.68\%)      & 18/478 (3.76\%)     & 35/486 (7.20\%)      & 18/252 (7.14\%)\\
                                      & Unseen &  2/6319 (0.31\%)         & 359/6317 (5.68\%)   & 113/2465 (4.58\%)    & 102/1591 (6.41\%)   & 91/1414 (6.43\%)     & 53/847 (6.25\%)  \\
                                      & All   & 2/8294 (0.024\%)         & 458/8292 (5.52\%)   & 141/3224 (4.37\%)    & 120/2069 (5.79\%)  & 126/1900 (6.63\%)   & 71/1099 (6.46\%) \\
        \hline
        \end{tabular}
        \caption{Inconsistency analysis on \textbf{CNET-ImDb}. Entity with a single mention are ignored}
    \end{subtable}

   


==> tables/rotoWire_removeFirst_santence_results.tex <==
    \begin{subtable}{1\textwidth}
     \centering

    \begin{tabular}{lccccc}
    \hline
    \textbf{Label} & \textbf{Model} & \textbf{Set} & \textbf{Precision} & \textbf{Recall}& \textbf{F1}  \\
    \hline
        \multirow{8}{*}{Looser} & \multirow{4}{*}{Baseline}     & Seen        & 0.76 (-5) & \textbf{0.72} (-5) & 0.74 (-5) \\
                                 &                              & Seen/Unseen & 0.72 (-5) & \textbf{0.72} (-2) & \textbf{0.72} (-3)\\
                                 &                              & Unseen      & 0.70 (-6) & \textbf{0.71} (-2) & \textbf{0.71} (-3)\\
                                 &                              & All         & 0.72 (-5) & \textbf{0.72} (-2) & 0.72 (-4)\\
                                 \cline{2-6}
                                 & \multirow{4}{*}{BaselineCLS} & Seen        & \textbf{0.81} (-8) & \textbf{0.72} (+6) & \textbf{0.76} (-1) \\
                                 &                              & Seen/Unseen & \textbf{0.75} (-9) & 0.70 (+9)         & \textbf{0.72} (+1) \\
                                 &                              & Unseen      & \textbf{0.74} (-11) & 0.66 (+8)         & 0.70 (+2) \\
                                 &                              & All         & \textbf{0.76} (-9) & 0.70 (+9)         & \textbf{0.73} (+2)  \\
                                \cline{2-6} 
        \multirow{8}{*}{Winner}  & \multirow{4}{*}{Baseline}    & Seen        & 0.76 (-4)          & \textbf{0.72} (-14) & 0.74 (-8)\\
                                 &                              & Seen/Unseen & \textbf{0.76} (-2) & 0.76 (-5)          & 0.76 (-3)\\
                                 &                              & Unseen      & 0.76 (-2)          & 0.80 (-1)          & 0.78 (-1)\\
                                 &                              & All         & \textbf{0.76}(-3)  & 0.76 (-5)          & 0.76 (-4)\\
                                \cline{2-6}
                                 & \multirow{4}{*}{BaselineCLS} & Seen        & \textbf{0.81} (+6) & \textbf{0.72} (-20) & \textbf{0.76} (-7)\\
                                 &                              & Seen/Unseen & 0.75          (+2) & \textbf{0.80} (-10) & \textbf{0.78} (-3)\\
                                 &                              & Unseen      & \textbf{0.77} (-5) & \textbf{0.85} (-6) & \textbf{0.81} (0)\\
                                 &                              & All         & 0.75          (+2) & \textbf{0.81} (-10) & \textbf{0.78} (-3)\\        

    \hline
    \end{tabular}
    \caption{Label statistics on rotowire}
    \end{subtable}
   \begin{subtable}{0.5\textwidth}
   \centering
    \begin{tabular}{lccc}
    \hline
    \textbf{Model} & \textbf{Set} & \textbf{BCELoss} & \textbf{Accurary}   \\
    \hline
        \multirow{4}{*}{Baseline}   & Seen        & 0.563\pm0.016 (+0.006) & 0.799\pm0.006 ()  \\
                                    & Seen/Unseen & 0.663\pm0.021 (+0.040) & 0.768\pm0.006 ()  \\
                                    & Unseen      & 0.701\pm0.025 (-0.016) & 0.760\pm0.004 ()  \\
                                    & All         & 0.648\pm0.021 (+0.032) & 0.773\pm0.005 ()  \\
                                 \hline
        \multirow{4}{*}{BaselineCLS}  & Seen        & \textbf{0.522}\pm0.023 () & \textbf{0.820}\pm0.002 () \\
                                      & Seen/Unseen & \textbf{0.589}\pm0.018 () & \textbf{0.787}\pm0.003 () \\
                                      & Unseen      & \textbf{0.604}\pm0.022 () & \textbf{0.785}\pm0.007 () \\
                                      & All         & \textbf{0.579}\pm0.020 () & \textbf{0.792}\pm0.002 () \\

    \hline
    \end{tabular}
        \caption{Overall statistics on rotowire}

    \end{subtable}
   


==> tables/roto_results_small.tex <==
     %\centering
    \footnotesize
\begin{tabular}{|c|c||c|c|}
\hline
\multirow{3}{*}{\textbf{Models}}& \multirow{3}{*}{\textbf{Set}} & \multicolumn{2}{c|}{\mu F1}                       \\
                                &                               & CNET                    & CNER                \\
                            
                                
\hline
\multirow{4}{*}{BERT-Linear}    & Seen                           &  0.44       & 0.51      \\
                                & Seen/Unseen                    &  0.43       & 0.49      \\
                                & Unseen                          &  0.44       & 0.48      \\
\hline
\multirow{4}{*}{BERT-CLS}       & Seen                          &  0.39       & 0.47   \\
                                & Seen/Unseen                    &  0.38       & 0.44    \\
                                & Unseen                         &  0.36       & 0.41       \\
\hline
\multirow{4}{*}{BERT-CRF}       & Seen                          & -   & 0.60   \\
                                & Seen/Unseen                   & -    & 0.53      \\
                                & Unseen                        & -    & 0.49    \\
\hline
\multirow{4}{*}{BERT-CLS-CRF}   & Seen                          & -   & 0.53       \\
                                & Seen/Unseen                   & -   & 0.48    \\
                                & Unseen                        & -   & 0.45      \\


\hline
\end{tabular}


==> tables/roto_task2_results.tex <==
     \centering
    \footnotesize
\begin{tabular}{|c|c||ccc|ccc|c||ccc|ccc|ccc|c|}
\hline
\multirow{3}{*}{\textbf{Models}}& \multirow{3}{*}{\textbf{Set}} & \multicolumn{7}{c||}{CNET}                                                & \multicolumn{10}{c|}{CNER}          \\
\cline{3-19}
                                &                               & \multicolumn{3}{c}{Winner}         & \multicolumn{3}{c}{Looser} & All    &  \multicolumn{3}{c}{Entity} &  \multicolumn{3}{c}{Looser} & \multicolumn{3}{c}{Winner} & All   \\ 
                                &                               & P         & R             &  F1    & P         & R      & F1    & \mu F1 &  P         & R      & F1    &  P         & R      & F1    & P         & R      & F1    & \mu F1 \\
\hline
\multirow{4}{*}{BERT-Linear}    & Seen                          &  0.84     &  0.78         &  0.81  & 0.76      & 0.82   &  0.79 &  0.81  &  0.82      &  0.91  & 0.86  &  0.58      &  0.72  & 0.63  &  0.70     & 0.66   &  0.68 &  0.66     \\
                                & Seen/Unseen                   &  0.85     &  0.79         &  0.82  & 0.78      & 0.83   &  0.8  &  0.81  &  0.81      &  0.89  & 0.85  &  0.58      &  0.70  & 0.63  &  0.68     & 0.68   &  0.68 &  0.65      \\
                                & Unseen                        &  0.84     &  0.78         &  0.81  & 0.75      & 0.82   &  0.78 &  0.80  &  0.76      &  0.87  & 0.81  &  0.54      &  0.67  & 0.58  &  0.68     & 0.68   &  0.68 &  0.63       \\
\hline
\multirow{4}{*}{BERT-CLS}       & Seen                          & 0.82      & 0.83          & 0.82   & 0.80      & 0.79   & 0.80  &  0.81  &  0.85      &  0.91  & 0.88  &   0.60     & 0.67   &  0.63 &  0.70     &  0.72  &  0.71 &  0.67   \\
                                & Seen/Unseen                   & 0.83      & 0.83          & 0.83   & 0.80      & 0.79   & 0.80  &  0.81  &  0.83      &  0.90  & 0.87  &  0.62      & 0.65   &  0.63 &  0.68     & 0.75   &  0.71 &  0.68    \\
                                & Unseen                        & 0.83      & 0.80          & 0.81   & 0.77      & 0.80   & 0.78  &  0.80  &  0.81      &  0.89  & 0.85  &   0.59     & 0.62   &  0.60 &   0.69    & 0.76   &  0.72 &  0.67       \\
\hline
\multirow{4}{*}{BERT-CRF}       & Seen                          & -         & -             & -      & -         & -      & -     & -      &  0.93      &  0.87  & 0.90  &  0.66      &  0.66  &  0.66 &  0.74     & 0.63   &  0.68 &  0.67   \\
                                & Seen/Unseen                   & -         & -             & -      & -         & -      & -     & -      &  0.92      &  0.85  & 0.88  & 0.67       &  0.63  &  0.65 &  0.73     & 0.66   &  0.69 &  0.67      \\
                                & Unseen                        & -         & -             & -      & -         & -      & -     & -      &  0.91      &  0.83  & 0.87  &  0.66      &  0.58  &  0.62 &  0.73     &  0.67  &  0.70 &  0.66    \\
\hline
\multirow{4}{*}{BERT-CLS-CRF}   & Seen                          & -         & -             & -      & -         & -      & -     & -      &  0.76      &  0.92  & 0.82  &  0.56      &  0.66  & 0.59  &  0.63     &  0.70  &  0.65 &  0.61       \\
                                & Seen/Unseen                   & -         & -             & -      & -         & -      & -     & -      &  0.75      &  0.89  & 0.81  &  0.56      &  0.64  & 0.58  &  0.62     &  0.69  &  0.65 &  0.61     \\
                                & Unseen                        & -         & -             & -      & -         & -      & -     & -      &  0.74      & 0.87   & 0.79  &  0.55      &  0.60  & 0.56  &  0.62     &  0.69  &  0.64 &  0.60       \\


\hline
\end{tabular}



==> tables/rotowire_randomMasking_results.tex <==
    \begin{subtable}{1\textwidth}
     \centering

    \begin{tabular}{lccccc}
    \hline
    \textbf{Label} & \textbf{Model} & \textbf{Set} & \textbf{Precision} & \textbf{Recall}& \textbf{F1}  \\
    \hline
        \multirow{8}{*}{Looser} & \multirow{4}{*}{Baseline}     & Seen        & 0.83         & 0.78         & 0.81 \\
                                 &                              & Seen/Unseen & \textbf{0.79} & \textbf{0.75} & \textbf{0.77} \\
                                 &                              & Unseen      & \textbf{0.79} & \textbf{0.73} & \textbf{0.76} \\
                                 &                              & All         & 0.79         & 0.75         & \textbf{0.77 \\
                                 \cline{2-6}
                                 & \multirow{4}{*}{BaselineCLS} & Seen        & \textbf{0.84} & \textbf{0.80} & \textbf{0.82} \\
                                 &                              & Seen/Unseen & \textbf{0.79} & \textbf{0.75} & \textbf{0.77} \\
                                 &                              & Unseen      & 0.76         & \textbf{0.73} & 0.75 \\
                                 &                              & All         & \textbf{0.80} & \textbf{0.76} & \textbf{0.78} \\
                                \cline{2-6} 
        \multirow{8}{*}{Winner}  & \multirow{4}{*}{Baseline}    & Seen        & 0.82         & 0.86         & 0.84 \\
                                 &                              & Seen/Unseen & \textbf{0.79} & \textbf{0.83} & \textbf{0.81} \\
                                 &                              & Unseen      & \textbf{0.79} & \textbf{0.84} & \textbf{0.81} \\
                                 &                              & All         & \textbf{0.80} & \textbf{0.83} & 0.81 \\
                                \cline{2-6}
                                 & \multirow{4}{*}{BaselineCLS} & Seen        & \textbf{0.83} & \textbf{0.87} & \textbf{0.85} \\
                                 &                              & Seen/Unseen & \textbf{0.79} & \textbf{0.83} & \textbf{0.81} \\
                                 &                              & Unseen      & 0.78         & 0.81         & 0.80 \\
                                 &                              & All         & \textbf{0.80} & \textbf{0.83} & \textbf{0.82}\\        

    \hline
    \end{tabular}
    \caption{Label statistics on rotowire}
    \end{subtable}
   \begin{subtable}{0.5\textwidth}
   \centering
    \begin{tabular}{lccc}
    \hline
    \textbf{Model} & \textbf{Set} & \textbf{BCELoss} & \textbf{Accurary}   \\
    \hline
        \multirow{4}{*}{Baseline}   & Seen        & 0.508\pm0.023 & 0.836\pm0.007  \\
                                    & Seen/Unseen & 0.637\pm0.031 & 0.802\pm0.008  \\
                                    & Unseen      & 0.654\pm0.048 & 0.796\pm0.011  \\
                                    & All         & 0.615\pm0.031 & 0.808\pm0.007  \\
                                 \hline
        \multirow{4}{*}{BaselineCLS}  & Seen        & \textbf{0.403}\pm0.036 & \textbf{0.865}\pm0.015 \\
                                      & Seen/Unseen & \textbf{0.521}\pm0.031 & \textbf{0.827}\pm0.012 \\
                                      & Unseen      & \textbf{0.535}\pm0.033 & \textbf{0.820}\pm0.012 \\
                                      & All         & \textbf{0.502}\pm0.031 & \textbf{0.833}\pm0.013 \\

    \hline
    \end{tabular}
        \caption{Overall statistics on rotowire}

    \end{subtable}
   


==> tables/task1_results_template.tex <==
    \begin{subtable}{1\textwidth}
     \centering

    \begin{tabular}{lccccc}
    \hline
    \textbf{Label} & \textbf{Model} & \textbf{Set} & \textbf{Precision} & \textbf{Recall}& \textbf{F1}  \\
    \hline
        \multirow{8}{*}{Looser} & \multirow{4}{*}{Baseline}     & Seen        &  &  &  \\
                                 &                              & Seen/Unseen &  &  &  \\
                                 &                              & Unseen      &  &  &  \\
                                 &                              & All         &  &  &  \\
                                 \cline{2-6}
                                 & \multirow{4}{*}{BaselineCLS} & Seen        &  &  &  \\
                                 &                              & Seen/Unseen &  &  &  \\
                                 &                              & Unseen      &  &  &  \\
                                 &                              & All         &  &  &  \\
                                \cline{2-6} 
        \multirow{8}{*}{Winner}  & \multirow{4}{*}{Baseline}    & Seen        &  &  &  \\
                                 &                              & Seen/Unseen &  &  &  \\
                                 &                              & Unseen      &  &  &  \\
                                 &                              & All         &  &  &  \\
                                \cline{2-6}
                                 & \multirow{4}{*}{BaselineCLS} & Seen        &  &  &  \\
                                 &                              & Seen/Unseen &  &  &  \\
                                 &                              & Unseen      &  &  &  \\
                                 &                              & All         &  &  &  \\        

    \hline
    \end{tabular}
    \caption{Label statistics on rotowire}
    \end{subtable}
   \begin{subtable}{0.5\textwidth}
   \centering
    \begin{tabular}{lccc}
    \hline
    \textbf{Model} & \textbf{Set} & \textbf{BCELoss} & \textbf{Accurary}   \\
    \hline
        \multirow{4}{*}{Baseline}   & Seen        & \pm & \pm  \\
                                    & Seen/Unseen & \pm & \pm  \\
                                    & Unseen      & \pm & \pm  \\
                                    & All         & \pm & \pm  \\
                                 \hline
        \multirow{4}{*}{BaselineCLS}  & Seen        & \pm & \pm \\
                                      & Seen/Unseen & \pm & \pm \\
                                      & Unseen      & \pm & \pm \\
                                      & All         & \pm & \pm \\

    \hline
    \end{tabular}
        \caption{Overall statistics on rotowire}

    \end{subtable}
   


==> tables/task2_imdb_results.tex <==
    \begin{subtable}{0.5\textwidth}
     \centering
\footnotesize
    \begin{tabular}{lccccc}
    \hline
    \textbf{Label} & \textbf{Model} & \textbf{Set} & \textbf{Precision} & \textbf{Recall}& \textbf{F1}  \\
    \hline
        \multirow{8}{*}{1}       & \multirow{4}{*}{Baseline}    & Seen        & 0.81 & 0.29 & 0.43 \\
                                 &                              & Unseen      & 0.73 & 0.25 & 0.38 \\
                                 &                              & All         & 0.74 & 0.26 & 0.39 \\
                                 \cline{2-6}
                                 & \multirow{4}{*}{BaselineCLS} & Seen        & 0.84 & 0.31 & 0.45 \\
                                 &                              & Unseen      & 0.69 & 0.25 & 0.37 \\
                                 &                              & All         & 0.71 & 0.26 & 0.38 \\
                                \cline{1-6} 
        \multirow{8}{*}{2}  & \multirow{4}{*}{Baseline}         & Seen        & 0.62 & 0.19 & 0.29 \\
                                 &                              & Unseen      & 0.43 & 0.13 & 0.20 \\
                                 &                              & All         & 0.46 & 0.14 & 0.22 \\
                                \cline{2-6}
                                 & \multirow{4}{*}{BaselineCLS} & Seen        & 0.64 & 0.17 & 0.27 \\
                                 &                              & Unseen      & 0.38 & 0.10 & 0.16 \\
                                 &                              & All         & 0.42 & 0.11 & 0.18 \\       
                                \cline{1-6}
        \multirow{8}{*}{3}  & \multirow{4}{*}{Baseline}         & Seen        & 0.55 & 0.12 & 0.20 \\
                                 &                              & Unseen      & 0.37 & 0.07 & 0.12 \\
                                 &                              & All         & 0.40 & 0.08 & 0.13 \\
                                \cline{2-6}
                                 & \multirow{4}{*}{BaselineCLS} & Seen        & 0.62 & 0.13 & 0.21 \\
                                 &                              & Unseen      & 0.35 & 0.07 & 0.12 \\
                                 &                              & All         & 0.39 & 0.08 & 0.13 \\       
                                \cline{1-6}
        \multirow{8}{*}{4}  & \multirow{4}{*}{Baseline}         & Seen        & 0.40 & 0.11 & 0.18 \\
                                 &                              & Unseen      & 0.16 & 0.04 & 0.06 \\
                                 &                              & All         & 0.20 & 0.05 & 0.08 \\
                                \cline{2-6}
                                 & \multirow{4}{*}{BaselineCLS} & Seen        & 0.56 & 0.12 & 0.20 \\
                                 &                              & Unseen      & 0.23 & 0.04 & 0.08 \\
                                 &                              & All         & 0.29 & 0.06 & 0.10 \\       
                                \cline{1-6}
        \multirow{8}{*}{Entity}  & \multirow{4}{*}{Baseline}    & Seen        & 0.64 & 0.19 & 0.29 \\
                                 &                              & Unseen      & 0.50 & 0.14 & 0.22 \\
                                 &                              & All         & 0.52 & 0.15 & 0.23 \\
                                \cline{2-6}
                                 & \multirow{4}{*}{BaselineCLS} & Seen        & 0.70 & 0.19 & 0.30 \\
                                 &                              & Unseen      & 0.47 & 0.13 & 0.20 \\
                                 &                              & All         & 0.51 & 0.14 & 0.22 \\

    \hline
    \end{tabular}
    \caption{Label statistics on CNER-ImDB}
    \end{subtable}
      \begin{subtable}{0.5\textwidth}
     \centering
    \footnotesize
    \begin{tabular}{lccc}
    \hline
    \textbf{Model} & \textbf{Set} & \textbf{BCELoss}    \\
    \hline
        \multirow{4}{*}{Baseline}   & Seen        & 0.220\pm0.015  \\
                                    & Unseen      & 0.404\pm0.029   \\
                                    & All         & 0.374\pm0.021   \\
                                 \hline
        \multirow{4}{*}{BaselineCLS}  & Seen        & 0.212\pm0.015  \\
                                      & Unseen      & 0.385\pm0.011  \\
                                      & All         & 0.356\pm0.009  \\

    \hline
    \end{tabular}
        \caption{Overall statistics on  CNER-ImDB}

    \end{subtable}
   


==> tables/task_2_result_template.tex <==
    \begin{subtable}{1\textwidth}
     \centering

    \begin{tabular}{lccccc}
    \hline
    \textbf{Label} & \textbf{Model} & \textbf{Set} & \textbf{Precision} & \textbf{Recall}& \textbf{F1}  \\
    \hline
        \multirow{8}{*}{1}       & \multirow{4}{*}{Baseline}    & Seen        & 0.81 & 0.29 & 0.43 \\
                                 &                              & Unseen      & 0.73 & 0.25 & 0.38 \\
                                 &                              & All         & 0.74 & 0.26 & 0.39 \\
                                 \cline{2-6}
                                 & \multirow{4}{*}{BaselineCLS} & Seen        & 0.84 & 0.31 & 0.45 \\
                                 &                              & Unseen      & 0.69 & 0.25 & 0.37 \\
                                 &                              & All         & 0.71 & 0.26 & 0.38 \\
                                \cline{1-6} 
        \multirow{8}{*}{2}  & \multirow{4}{*}{Baseline}         & Seen        & 0.62 & 0.19 & 0.29 \\
                                 &                              & Unseen      & 0.43 & 0.13 & 0.20 \\
                                 &                              & All         & 0.46 & 0.14 & 0.22 \\
                                \cline{2-6}
                                 & \multirow{4}{*}{BaselineCLS} & Seen        & 0.64 & 0.17 & 0.27 \\
                                 &                              & Unseen      & 0.38 & 0.10 & 0.16 \\
                                 &                              & All         & 0.42 & 0.11 & 0.18 \\       
                                \cline{1-6}
        \multirow{8}{*}{3}  & \multirow{4}{*}{Baseline}         & Seen        & 0.55 & 0.12 & 0.20 \\
                                 &                              & Unseen      & 0.37 & 0.07 & 0.12 \\
                                 &                              & All         & 0.40 & 0.08 & 0.13 \\
                                \cline{2-6}
                                 & \multirow{4}{*}{BaselineCLS} & Seen        & 0.62 & 0.13 & 0.21 \\
                                 &                              & Unseen      & 0.35 & 0.07 & 0.12 \\
                                 &                              & All         & 0.39 & 0.08 & 0.13 \\       
                                \cline{1-6}
        \multirow{8}{*}{4}  & \multirow{4}{*}{Baseline}         & Seen        & 0.40 & 0.11 & 0.18 \\
                                 &                              & Unseen      & 0.16 & 0.04 & 0.06 \\
                                 &                              & All         & 0.20 & 0.05 & 0.08 \\
                                \cline{2-6}
                                 & \multirow{4}{*}{BaselineCLS} & Seen        & 0.56 & 0.12 & 0.20 \\
                                 &                              & Unseen      & 0.23 & 0.04 & 0.08 \\
                                 &                              & All         & 0.29 & 0.06 & 0.10 \\       
                                \cline{1-6}
        \multirow{8}{*}{Entity}  & \multirow{4}{*}{Baseline}    & Seen        & 0.64 & 0.19 & 0.29 \\
                                 &                              & Unseen      & 0.50 & 0.14 & 0.22 \\
                                 &                              & All         & 0.52 & 0.15 & 0.23 \\
                                \cline{2-6}
                                 & \multirow{4}{*}{BaselineCLS} & Seen        & 0.70 & 0.19 & 0.30 \\
                                 &                              & Unseen      & 0.47 & 0.13 & 0.20 \\
                                 &                              & All         & 0.51 & 0.14 & 0.22 \\

    \hline
    \end{tabular}
    \caption{Label statistics on rotowire}
    \end{subtable}
   \begin{subtable}{0.5\textwidth}
   \centering
    \begin{tabular}{lccc}
    \hline
    \textbf{Model} & \textbf{Set} & \textbf{BCELoss}    \\
    \hline
        \multirow{4}{*}{Baseline}   & Seen        & 0.220\pm0.015  \\
                                    & Unseen      & 0.404\pm0.029   \\
                                    & All         & 0.374\pm0.021   \\
                                 \hline
        \multirow{4}{*}{BaselineCLS}  & Seen        & 0.212\pm0.015  \\
                                      & Unseen      & 0.385\pm0.011  \\
                                      & All         & 0.356\pm0.009  \\

    \hline
    \end{tabular}
        \caption{Overall statistics on rotowire}

    \end{subtable}
   

